Direct Assembly of Magnetic Janus Particles at a Droplet Interface

Self-assembly of nanoparticles at fluid-fluid interfaces is a promising route to fabricate functional materials from the bottom-up. However, directing and controlling particles into highly tunable and predictable structures -- while essential -- is a challenge. We present a liquid interface assisted approach to fabricate nanoparticle structures with tunable properties. To demonstrate its feasibility, we study magnetic Janus particles adsorbed at the interface of a spherical droplet placed on a substrate. With an external magnetic field turned on, a single particle moves to the location where its position vector relative to the droplet centre is parallel to the direction of the applied field. Multiple magnetic Janus particles arrange into reconfigurable hexagonal lattice structures and can be directed to assemble at desirable locations on the droplet interface by simply varying the magnetic field direction. We develop an interface energy model to explain our observations, finding excellent agreement. Finally, we demonstrate that the external magnetic field allows \revisedtext{one} to tune the particle deposition pattern obtained when the droplet evaporates. Our results have implications for the fabrication of varied nanostructures on substrates for use in nanodevices, organic electronics, or advanced display, printing and coating applications.

==> draw-janus-90degree.tex <==
\begin{figure}[htbp]
% \begin{center}
\begin{subfigure}{0.45\textwidth}
% \centering
 \begin{tikzpicture}
% 	\fill[white,opacity=0.4] (-4,-3) rectangle (4.0,0.0);
	\fill[white,opacity=0.4] (-4,0) rectangle (4.0,3.0);
	\draw[dashed] (-4,0) to (4,0);
% droplet	
\draw (-4,0) arc (180:0:4.0);
\node at (-2.0,0.5+1.0) [fontscale=4] {fluid $1$};
\node at (-2.0,2.5+1.7) [fontscale=4] {fluid $2$};
% janus half
	 \filldraw[fill=blue!60!white, draw=green!50!black]
         (2.4,1.5+1.7) -- (2.744,1.25+1.7) arc (-30-1:145-5:0.42) -- (2.4,1.5+1.7);
%janus half         
      \filldraw[fill=red!60!white, draw=green!50!black]
      (2.4,1.5+1.7) -- (2.04,1.72+1.7) arc (145:325:0.42) -- (2.4,1.5+1.7);
       
       \draw[ultra thick, black,arrows=->, >=stealth] (0.0,0) to (0.0,1.0);
	 \node at (-0.2,0.5) [fontscale=4] {$z$};
	 \draw[ultra thick, black,arrows=->,>=stealth] (0.0,0) to (-1.0,0.0);
	 \node at (-0.5,0.2) [fontscale=4] {$r$};
	
	
  	%dipole 
   	\draw[ultra thick, black,arrows=->,>=stealth] (2.4,1.5+1.7) to (2.744,2.05+1.7);
  	  \node at (2.7,2.3+1.7) [fontscale=4] {$\mathbf{m}$};
  	  
\node at (0.3,0.3) [fontscale=4] {$O$};
  %substrate
%  \draw[ultra thick, black] (-4.0,0.0) to (4.0,0.0);
 \fill[red,opacity=0.5] (-4.0,-0.4) rectangle (4.0,0.0);
  \fill[blue,opacity=0.5] (-4.5,-0.4) rectangle (-4.0,0.0);
  \fill[blue,opacity=0.5] (4.0,-0.4) rectangle (4.5,0.0);
  \draw[step=2mm, black] (-4.5,-0.4) grid (4.5,0.0);
           
%            \draw (1.0,-1.3) to (0.6,-1.5);
           
%          \draw[dashed] (0.0,-2.3) to (2.744,1.25);
         
%           \node at (1.7,1.25+1.7)[fontscale=4] {apolar};
%            \node at (3.0,1.72+1.5) [fontscale=4]{polar};

\end{tikzpicture}
% \caption{}
\label{fig:equi}
\end{subfigure}
 \hfill%
\begin{subfigure}{.45\textwidth}
 \begin{tikzpicture}
% 	\fill[white,opacity=0.4] (-4,-3) rectangle (4.0,0.0);
	\fill[white,opacity=0.4] (-4,0) rectangle (4.0,3.0);
	
	 \filldraw[fill=blue!60!white, draw=green!50!black]
         (2.4,1.5+1.7) -- (2.82,1.5+1.7) arc (0:150:0.42) -- (2.4,1.5+1.7);
 	 \filldraw[fill=blue!30!white, draw=green!50!black]
         (2.4,1.5+1.7) -- (2.04,1.72+1.7) arc (140:185:0.30) -- (2.4,1.5+1.7);
         
      \filldraw[fill=red!60!white, draw=green!50!black]
      (2.4,1.5+1.7) -- (1.98,1.5+1.7) arc (180:325:0.42) -- (2.4,1.5+1.7);
      
      	 \filldraw[fill=red!30!white, draw=green!50!black]
         (2.4,1.5+1.7) -- (2.744,1.25+1.7) arc (-30:0:0.49) -- (2.4,1.5+1.7);
         
	\draw (-4,0) arc (180:0:4.0);
	
	\draw[dashed] (-4,0) to (4,0);
	%magnetic field
	\draw[ultra thick, black,arrows=->,>=stealth] (-2.0,-1.0+1.7) to (-2.0,1.0+1.7);
	\node at (-1.5,0.5+1.7) [fontscale=4] {$\mathbf{H}$};
    
  	%dipole 
   	\draw[ultra thick, black,arrows=->,>=stealth] (2.4,1.5+1.7) to (2.4,2.2+1.7);
  	  \node at (2.7,2.3+1.7) [fontscale=4] {$\mathbf{m}$};
  	
%    	\draw[ultra thick,dashed,black,arrows=->,arrowhead=50cm,line width=2pt,>=stealth] (0,0.0) to (0,4.0);
%    	\draw[-{>[scale=3.0]}] (0,0.0) to (0,4.0);
\draw [ultra thick,dashed,black, decoration={markings,mark=at position 1 with
    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,0.0) to (0,4.0);
  	\node at (0.3,1.0+1.7) [fontscale=4] {$\mathbf{r_0}$};
        \node at (0.2,-1.3+1.9) [fontscale=4] {$\phi$};
        %angle beta
%          \draw[ultra thick,dashed,black,arrows=->,line width=2pt] (0.0,0.0) to (2.4,1.5+1.7);
         \draw [ultra thick,dashed,black, decoration={markings,mark=at position 1 with
    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0.0,0.0) to (2.4,1.5+1.7);
            \node at (1.5,0.5+2.0) [fontscale=4] {$\mathbf{r_i}$};
         %            \node at (1.2,-1.3) [fontscale=2] {$\beta$};

%            \draw (1.0,-1.3) to (0.6,-1.5);
%          \draw[dashed] (0.0,-2.3) to (2.744,1.25);
         
%           \node at (3.0,1.35)  {$A_{a2}$};
%            \node at (1.8,1.72)  {$A_{p1}$};
% \node at (0.3,0.3) [fontscale=4] {$O$};
  %substrate
%  \draw[ultra thick, black] (-4.0,0.0) to (4.0,0.0);
 \fill[red,opacity=0.5] (-4.0,-0.4) rectangle (4.0,0.0);
  \fill[blue,opacity=0.5] (-4.5,-0.4) rectangle (-4.0,0.0);
  \fill[blue,opacity=0.5] (4.0,-0.4) rectangle (4.5,0.0);
  \draw[step=2mm, black] (-4.5,-0.4) grid (4.5,0.0);

\end{tikzpicture}
\caption{}
\label{fig:tilt}
\end{subfigure}
% \end{center}
\caption{A single Janus particle adsorbed at a droplet interface in its
equilibrium orientation $(a)$ and under vertical magnetic field $(b)$. The Janus
particle consists of an apolar and a polar hemisphere.  The particle's magnetic
dipole moment $\mathbf{m}$ is orthogonal to the Janus boundary, and the
external magnetic field, $\mathbf{H}$, is directed upward.
The angle $\varphi$ is defined as the angle between droplet center to droplet top vector $\mathbf{r_0}$ and droplet center to particel center vector $\mathbf{r_i}$.}
% $A_{a2}$ and $A_{p1}$ are the surface areas of the apolar hemisphere immersed in fluid $2$ and the polar hemisphere immersed in fluid $1$, respectively.}
\label{fig:janus-geo}
\end{figure}

==> multi-particles.tex <==
% \section{Theory and simulation results}
% \emph{Results}\textemdash{}
% \subsection{Multiple particles}

\textbf{Multiple magnetic Janus particles.}
%
% \subsection{Multiple janus particle}
Having obtained a good understanding of the behaviour of a single magnetic Janus particle adsorbed at a surface droplet interface, we investigate the self-assembly of multiple magnetic Janus particles.
Starting from a random initial placement
of $3$ magnetic Janus particles adsorbed at the interface, we let
the system reach the steady-state. We then add one more particle at the droplet interface, let the system reach steady state again and repeat this process for up to $N=6$ particles. 
We show the structures obtained in \figref{p36-snap} for a given number of particles.
\begin{figure}[htbp]
% \centering
 \begin{subfigure}{.2\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p3.pdf}
 \subcaption{}
 \label{fig:p3}
\end{subfigure}
% \caption{Snapshots of assembled structures during drying magnetic Janus particle suspension droplet.}
\hspace{1mm}
 \begin{subfigure}{.2\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p4.pdf}
 \subcaption{}
 \label{fig:p4}
\end{subfigure}
\\
\begin{subfigure}{.2\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p5.pdf}
 \subcaption{}
 \label{fig:p5}
 \end{subfigure}
 \hspace{1mm}
\begin{subfigure}{.2\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p6.pdf}
 \subcaption{}
 \label{fig:p6}
 \end{subfigure}
 
\caption{Clusters observed in simulations for $N=3-6$ particles with
amphiphilicty $\beta=30^{\circ}$ and external dipole-field strength $B_m/\pi
a^2 \gamma_{12}=1.31$. The particles exhibit a hexagonal lattice-like
arrangement.}
\label{fig:p36-snap}
\end{figure}

$N=3$ particles arrange into a triangular lattice-like structure around the
droplet centre (\figref{p3}), instead of the straight chain-like configuration
found by magnetic Janus particles at flat fluid-fluid
interfaces.~\cite{Xie2016}  This structure is similar to the $3$-particle
structure observed for colloidal particles adsorbed at a liquid crystal droplet
interface~\cite{Rahimi2015} and for colloidal particles interacting with short
range-interactions.~\cite{Pine2003,Arkus2009}  For $N=4-6$ particles, we find
the particles all favour hexagonal arrangements (\figref{p4}, \figref{p5} and
\figref{p6}), which suggests the hexagonal arrangement may be the interface
energy minimum configuration for $N > 3$ particles. 

Applying our free energy model for a single particle to the case for $N$
particles with assuming that the magnetic dipole-dipole interactions between
the particles are negligible, the interface energy is:
\begin{equation}
 \Delta E_t = 4  a^2 \gamma_{12} \sin \beta \sum_{i}^{N} \phi_i
 \mbox{.}
\end{equation}

To estimate the total interface energy for the $3$-particle system, we fix two
particles next to each other, and move the third particle with the pair angle
$\varphi$ from $\varphi=0^{\circ}$ to $\varphi=120^{\circ}$, as illustrated in
the inset of~\figref{p3-energy}.  \figref{p3-energy} shows that the interface
energy decreases monotonically with increasing particle pair-pair angle
$\varphi$ and the interface energy becomes minimal at $\varphi=120^{\circ}$,
which represents a triangular arrangement, in agreement with simulation
results.
\begin{figure}[htbp]
% \centering
% \begin{subfigure}{.45\textwidth}
\includegraphics[width= 0.45\textwidth]{imgacsnano/p3-energy.pdf}
%  \subcaption{}
%  \label{fig:p3-energy}
%  \end{subfigure}
%  \hfill
\caption{Normalized interface energy $\Delta E_t/a^2 \gamma_{12} $ as a function
of particle pair-pair angle $\varphi$. The interface energy takes a minimum at
$\varphi = 120^{\circ}$, which represents a triangular lattice-like
arrangement, in agreement with our simulation results.}
\label{fig:p3-energy}
\end{figure}

For $N=4-6$ particles, it is nontrivial to estimate the interface energy as a
function of a single parameter, however, after some mathematical analysis we
find that minimising $\sum_{i}^{N} \phi_i$ is identical to minimising the total
particle-centre to droplet-centre distance $L = \sum_{i}^{N} |\mathbf{r}_i -
\mathbf{r}_0|$, with the following two constraints: $1)$ particles are located
at the droplet interface, $ |\mathbf{r}_i| =R $, and $2)$ particles do not
overlap, $|\mathbf{r}_i - \mathbf{r}_j| \geq 2a$.  In addition, in a strong
magnetic field, the orientation of the particle is fixed parallel to the
magnetic field direction and the particles are adsorbed at the droplet
interface, which leaves only two degrees of freedom for the particles.
Therefore, we can model our system as a quasi-$2D$ system.  Minimising $L$ for
spherical particles in a $2D$ system yields particles that conform to closest
packing, which is a hexagonal arrangement. Therefore, our theoretical model's
prediction that hexagonal arrangement is energetically favourable for
self-assembly of multiple magnetic Janus particles agrees with our simulation
results.

\textbf{Varying the magnetic field direction.}
With even more particles $N=40$, we investigate the relocation and
rearrangement of particles by varying the external field starting from pointing
vertically upward, to vertically downward and finally to left horizontal
direction. Under an upward magnetic field, the particles assemble at the top
of the droplet ordered in a hexagonal arrangement (\figref{p40-up-top} and
\figref{p40-up-side}). When we switch the magnetic field to the downward
direction, the particles rotate instantly by $180^{\circ}$, move immediately
downwards towards to the surface droplet contact line and finally align in a
ring-like structure at the edge of the droplet (\figref{p40-down-top} and
\figref{p40-down-side}). On switching the magnetic field to the left
horizontal direction, the particles rotate by $90^{\circ}$, move to the left side
of the droplet and form highly ordered layers (\figref{p40-left-top} and
\figref{p40-left-side}). [Movie S1]

Our simulations therefore show that it is possible to direct the particles to
assemble at desirable locations at the droplet interface based on the direction
of the external magnetic field, and that the final assembled structure is
tunable depending on the direction and magnitude of the applied magnetic field.
One can immediately forsee technological applications as \textit{e.g.,} a photonic
material or alternative to currently used electrophoretic/electronic inks (E-inks), where
electrophoretic particles encapsulated in a microdroplet are relocated by an
external electric field.~\cite{Comiskey1998}
\begin{figure}[htbp]
% \centering
\begin{subfigure}{.15\textwidth}
\includegraphics[width= 0.9\textwidth]{imgacsnano/p40-zup.pdf}
 \subcaption{upward $\mathbf{H}$ - top view}
 \label{fig:p40-up-top}
 \end{subfigure}
 \begin{subfigure}{.15\textwidth}
\includegraphics[width= 0.9\textwidth]{imgacsnano/p40-zdown-top.pdf}
 \subcaption{downward $\mathbf{H}$ - top view}
 \label{fig:p40-down-top}
 \end{subfigure}
 \begin{subfigure}{.15\textwidth}
\includegraphics[width= 0.9\textwidth]{imgacsnano/p40-zleft-top.pdf}
 \subcaption{left $\mathbf{H}$ - \\top view}
 \label{fig:p40-left-top}
 \end{subfigure}
\\
 \begin{subfigure}{.15\textwidth}
\includegraphics[width= 0.9\textwidth]{imgacsnano/p40-zup-side.pdf}
 \subcaption{upward $\mathbf{H}$ - side view}
 \label{fig:p40-up-side}
 \end{subfigure}
 \begin{subfigure}{.15\textwidth}
\includegraphics[width= 0.9\textwidth]{imgacsnano/p40-zdown-side.pdf}
 \subcaption{downward $\mathbf{H}$ - side view}
 \label{fig:p40-down-side}
 \end{subfigure}
 \begin{subfigure}{.15\textwidth}
\includegraphics[width= 0.9\textwidth]{imgacsnano/p40-zleft-side.pdf}
 \subcaption{left $\mathbf{H}$ -\\ side view}
 \label{fig:p40-left-side}
 \end{subfigure}
 
\caption{Snapshot of $N = 40$ particles adsorbed at a droplet interface with
amphiphilicty $\beta=30^{\circ}$ and dipole-field strength $B_m/\pi
a^2\gamma_{12}=1.31$ under different magnetic field directions. The particles
relocate and form different ordered structures depending on the direction of
the magnetic field.}
\label{fig:p40-snap}
\end{figure}

% \subsection{Particle deposition}
\textbf{Particle deposition during evaporation.}
Finally, we investigate the case of many magnetic Janus particles adsorbed at a
surface droplet interface that undergoes evaporation, a scenario that occurs
frequently in reality when coatings and paints dry. To simulate fluid
evaporation, we use a diffusion dominated evaporation model, developed recently
in our group.~\cite{DennisXieJens2016} The starting configuration of the system
before evaporation is the same as those shown in \textit{e.g.,} Fig~\ref{fig:p40-snap}.
Once a steady-state is reached, we start to evaporate the droplet.

When an upward magnetic field is applied, the particles stay at the top during
the evaporation of the droplet (\figref{p30-zup-1}).  The contact angle of the
droplet decreases until it reaches $30^{\circ}$, after which the contact lines
de-pins from the border of the hydrophilic area and moves towards the centre
(\figref{p30-zup-2}).  This is the well-known stick-slip
phenomenon,~\cite{Detlef2015} usually encountered during the evaporation of
droplets on a rough solid substrate.  After the contact line depins, the
droplet continues to dewet (\figref{p30-zup-3}) and approaches the geometry of
a planar film.  The Janus particle will deform the planar film in a monopolar
fashion, introducing attractive capillary forces between particles.  The
attractive capillary forces ensure close packing of the particles, and finally,
a dried highly ordered particle monolayer remains on the substrate
(\figref{p30-zup-4}). [Movie S2]

Under the influence of a downward magnetic field, the particles stay at the
edge of the droplet, forming a ring-like structure during the evaporation of
droplet (\figref{p30-zdown-1}).  The contact angle of the droplet continuously
decreases. We do not observe depinning behaviour once the contact angle reaches
$30^{\circ}$, in contrast with the behaviour observed for an upwardly directed
magnetic field. This is caused by self-pinning due to the particles confined at
the contact line. The colloidal particles experience friction with the
substrate, thus strengthening the pinning of the contact line on the substrate.
When the contact angle decreases further approaching zero degrees, the liquid
film begins to rupture at areas on the edge of the droplet
(\figref{p30-zdown-2}) and the droplet rapidly dries in these areas
(\figref{p30-zdown-3}).  Finally, after full evaporation, a ring-like particle
structure is deposited on the substrate (\figref{p30-zdown-4}). [Movie S3]

\begin{figure}[b!]
% \centering
\begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zup-1.pdf}
 \subcaption{}
 \label{fig:p30-zup-1}
 \end{subfigure}
 \begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zup-2.pdf}
 \subcaption{}
 \label{fig:p30-zup-2}
\end{subfigure}
\begin{subfigure}{.1\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zup-3.pdf}
 \subcaption{}
 \label{fig:p30-zup-3}
 \end{subfigure}
 \begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zup-5.pdf}
 \subcaption{}
 \label{fig:p30-zup-4}
\end{subfigure}

\begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zdown-1.pdf}
 \subcaption{}
 \label{fig:p30-zdown-1}
 \end{subfigure}
 \begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zdown-3.pdf}
 \subcaption{}
 \label{fig:p30-zdown-2}
\end{subfigure}
\begin{subfigure}{.1\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zdown-4.pdf}
 \subcaption{}
 \label{fig:p30-zdown-3}
 \end{subfigure}
 \begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zdown-5.pdf}
 \subcaption{}
 \label{fig:p30-zdown-4}
\end{subfigure}

\begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zleft-1.pdf}
 \subcaption{}
 \label{fig:p30-zleft-1}
 \end{subfigure}
 \begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zleft-3.pdf}
 \subcaption{}
 \label{fig:p30-zleft-2}
\end{subfigure}
\begin{subfigure}{.1\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zleft-4.pdf}
 \subcaption{}
 \label{fig:p30-zleft-3}
 \end{subfigure}
 \begin{subfigure}{.10\textwidth}
\includegraphics[width= 1.0\textwidth]{imgacsnano/p40-zleft-5.pdf}
 \subcaption{}
 \label{fig:p30-zleft-4}
\end{subfigure}

\caption{Snapshots of the assembled structures during droplet evaporation and with an
 upward (a)-(d), downward (e)-(h) and left horizontal (i)-(l) applied magnetic field. Influenced by an upward magnetic field (a-d), the particles remain at the top of the droplet while the contact line decreases before it de-pins. Under a downward magnetic field (e-h), the particles form a ring-like structure that self-pins the contact line, and the contact line deceases continuously. Finally, in a horizontal magnetic field (i-l) the particles migrate in the field direction and cause self-pinning on one side of the droplet, while the contact line recedes on the opposite side and causes inhomogeneous evaporation leading to looser particle arrangements.}
\label{fig:p30-snap}
\end{figure}

Under a left oriented horizontal magnetic field, the particles stay at the left
side of the droplet during the evaporation, as naively expected
(\figref{p30-zleft-1}).  The contact angle of the droplet continuously
decreases, and the contact line depins first at the right side where there is
no self-pinning due to the Janus particles (\figref{p30-zleft-2}). The contact
angle approaches zero degrees and the droplet geometry tends to that of a
planar film, similar to the case of an upwardly directed magnetic field.  In
contrast with the upwardly directed magnetic field, under a horizontal magnetic
field, the Janus particles deform the planar film in a dipolar
fashion~\cite{Xie2015,Xie2016}, and dipolar capillary interactions arise
(\figref{p30-zleft-3}).  This dipolar capillary force is repulsive between
neighbouring particles in the horizontal direction~\cite{Xie2016}, thus the
final structure shows a looser arrangement of particles (\figref{p30-zleft-4})
compared with the particle deposition formed in an upward magnetic field
(\figref{p30-zup-4}). [Movie S4]

Our results demonstrate that the direction of the magnetic field allows one to
tune the particle deposition pattern obtained due to the evaporation and drying
of a Janus particle-laden droplet, which \revisedtext{can find} potential applications in
e.g. advanced printing, electronics or display technology.




